Model Predictive Control of District Heating Grids Using Stabilizing Terminal Ingredients

The transformation of fossil fuel-based district heating grids (DHGs) to CO$_2$-neutral DHGs requires the development of novel operating strategies. Model predictive control (MPC) is a promising approach, as knowledge about future heat demand and heat supply can be incorporated into the control, operating constraints can be ensured and the stability of the closed-loop system can be guaranteed. In this paper, we employ MPC for DHGs to control the system mass flows and injected heat flows. Following common practice, we derive terminal ingredients to stabilize given steady state temperatures and storage masses in the DHG. To apply MPC with terminal ingredients, it is crucial that the system under control is stabilizable. By exploiting the particular system structure, we give a sufficient condition for the stabilizability in terms of the grid topology and hence, for the applicability of the MPC scheme to DHGs. Furthermore, we demonstrate the practicability of the application of MPC to an exemplary DHG in a numerical case study.

==> figures/networkUnits.tex <==
\newcommand{\HXlayerA}[2]{\begin{tikzpicture}[>=latex, line width=#2*.35mm,scale=#2]
    \draw[orange] (0,\dx) to[out=270,in=180] (\dr,\dx-\dr);

    \draw[orange] (\dr,\dx-\dr) -- (\dx-\dr,\dx-\dr);
    \draw[orange] (\dx-\dr,\dx-\dr) to[out=0,in=90] (\dx,\dx-2*\dr);
    \draw[orange] (\dx,\dx-2*\dr) to[out=270,in=0] (\dx-\dr,\dx-3*\dr);

    \draw[orange] (\dx-\dr,\dx-3*\dr) -- (-\dx+\dr,\dx-3*\dr);
    \draw[orange] (-\dx+\dr,\dx-3*\dr) to[out=180,in=90] (-\dx,\dx-4*\dr);
    \draw[orange] (-\dx,\dx-4*\dr) to[out=270,in=180] (-\dx+\dr,\dx-5*\dr);

    \draw[orange] (-\dx+\dr,\dx-5*\dr) -- (\dx-\dr,\dx-5*\dr);

    \draw[orange, path fading=south] (\dx-\dr,\dx-5*\dr) to[out=0,in=90] (\dx,\dx-6*\dr) to[out=270,in=0] (\dx-\dr,\dx-7*\dr);
    \draw[orange!50!blue, path fading=north] (\dx-\dr,\dx-5*\dr) to[out=0,in=90] (\dx,\dx-6*\dr) to[out=270,in=0] (\dx-\dr,\dx-7*\dr);
    \draw[orange!50!blue] (\dx-\dr,\dx-7*\dr) -- (-\dx+\dr,\dx-7*\dr);
    \draw[orange!50!blue, path fading=south] (-\dx+\dr,\dx-7*\dr) to[out=180,in=90] (-\dx,\dx-8*\dr) to[out=270,in=180] (-\dx+\dr,\dx-9*\dr);
    \draw[blue, path fading=north] (-\dx+\dr,\dx-7*\dr) to[out=180,in=90] (-\dx,\dx-8*\dr) to[out=270,in=180] (-\dx+\dr,\dx-9*\dr);
    
    \draw[blue] (-\dx+\dr,\dx-9*\dr) -- (\dx-\dr,\dx-9*\dr);
    \draw[blue] (\dx-\dr,\dx-9*\dr) to[out=0,in=90] (\dx,\dx-10*\dr);
    \draw[blue] (\dx,\dx-10*\dr) to[out=270,in=0] (\dx-\dr,\dx-11*\dr);

    \draw[blue] (\dx-\dr,\dx-11*\dr) -- (-\dx+\dr,\dx-11*\dr);
    \draw[blue] (-\dx+\dr,\dx-11*\dr) to[out=180,in=90] (-\dx,\dx-12*\dr);
    \draw[blue] (-\dx,\dx-12*\dr) to[out=270,in=180] (-\dx+\dr,\dx-13*\dr);

    \draw[blue] (-\dx+\dr,\dx-13*\dr) -- (-\dr,-\dx+\dr);
    \draw[blue] (-\dr,-\dx+\dr) to[out=0,in=90] (0,-\dx);
\end{tikzpicture}}

\newcommand{\TESlayerA}[2]{\begin{tikzpicture}[>=latex, line width=#2*.35mm,scale=#2]
	\coordinate (BL) at (-1.35*\dx,-2*\dx); 
    \coordinate (TL) at (-1.35*\dx,2*\dx);
    \coordinate (TR) at (1.35*\dx,2*\dx);
    \coordinate (BR) at (1.35*\dx,-2*\dx);

    \coordinate (BLinner) at (-1.35*\dx, -\dx); 
    \coordinate (BRinner) at (1.35*\dx, -\dx);

    \coordinate (TLinner) at (-1.35*\dx, \dx);
    \coordinate (TRinner) at (1.35*\dx, \dx);

    \draw[fill=blue] (BLinner) -- (BL) to[out=270,in=270] (BR) -- (BRinner);

    \draw[fill=orange] (TLinner) -- (TL) to[out=90,in=90] (TR) -- (TRinner);

    \filldraw[color=orange, fill = orange, path fading = south] (BRinner) -- (BLinner) -- (TLinner) -- (TRinner);
    \filldraw[color=blue, fill = blue, path fading = north] (BRinner) -- (BLinner) -- (TLinner) -- (TRinner);

    \draw[color=black] (-1.35*\dx, \dx+.1*\dx) -- (-1.35*\dx, -\dx-.1*\dx);
    \draw[color=black] (1.35*\dx, \dx+.1*\dx) -- (1.35*\dx, -\dx-.1*\dx);
\end{tikzpicture}}

\newcommand{\HXlayerB}[2]{\begin{tikzpicture}[>=latex, line width=#2*.35mm,scale=#2]
    \draw[red] (0,\dx) to[out=270,in=180] (\dr,\dx-\dr);

    \draw[red] (\dr,\dx-\dr) -- (\dx-\dr,\dx-\dr);
    \draw[red] (\dx-\dr,\dx-\dr) to[out=0,in=90] (\dx,\dx-2*\dr);
    \draw[red] (\dx,\dx-2*\dr) to[out=270,in=0] (\dx-\dr,\dx-3*\dr);

    \draw[red] (\dx-\dr,\dx-3*\dr) -- (-\dx+\dr,\dx-3*\dr);
    \draw[red] (-\dx+\dr,\dx-3*\dr) to[out=180,in=90] (-\dx,\dx-4*\dr);
    \draw[red] (-\dx,\dx-4*\dr) to[out=270,in=180] (-\dx+\dr,\dx-5*\dr);

    \draw[red] (-\dx+\dr,\dx-5*\dr) -- (\dx-\dr,\dx-5*\dr);

    \draw[red, path fading=south] (\dx-\dr,\dx-5*\dr) to[out=0,in=90] (\dx,\dx-6*\dr) to[out=270,in=0] (\dx-\dr,\dx-7*\dr);
    \draw[red!50!orange, path fading=north] (\dx-\dr,\dx-5*\dr) to[out=0,in=90] (\dx,\dx-6*\dr) to[out=270,in=0] (\dx-\dr,\dx-7*\dr);
    \draw[red!50!orange] (\dx-\dr,\dx-7*\dr) -- (-\dx+\dr,\dx-7*\dr);
    \draw[red!50!orange, path fading=south] (-\dx+\dr,\dx-7*\dr) to[out=180,in=90] (-\dx,\dx-8*\dr) to[out=270,in=180] (-\dx+\dr,\dx-9*\dr);
    \draw[orange, path fading=north] (-\dx+\dr,\dx-7*\dr) to[out=180,in=90] (-\dx,\dx-8*\dr) to[out=270,in=180] (-\dx+\dr,\dx-9*\dr);
    
    \draw[orange] (-\dx+\dr,\dx-9*\dr) -- (\dx-\dr,\dx-9*\dr);
    \draw[orange] (\dx-\dr,\dx-9*\dr) to[out=0,in=90] (\dx,\dx-10*\dr);
    \draw[orange] (\dx,\dx-10*\dr) to[out=270,in=0] (\dx-\dr,\dx-11*\dr);

    \draw[orange] (\dx-\dr,\dx-11*\dr) -- (-\dx+\dr,\dx-11*\dr);
    \draw[orange] (-\dx+\dr,\dx-11*\dr) to[out=180,in=90] (-\dx,\dx-12*\dr);
    \draw[orange] (-\dx,\dx-12*\dr) to[out=270,in=180] (-\dx+\dr,\dx-13*\dr);

    \draw[orange] (-\dx+\dr,\dx-13*\dr) -- (-\dr,-\dx+\dr);
    \draw[orange] (-\dr,-\dx+\dr) to[out=0,in=90] (0,-\dx);
\end{tikzpicture}}

\newcommand{\TESlayerB}[2]{\begin{tikzpicture}[>=latex, line width=#2*.35mm,scale=#2]
	\coordinate (BL) at (-1.35*\dx,-2*\dx); 
    \coordinate (TL) at (-1.35*\dx,2*\dx);
    \coordinate (TR) at (1.35*\dx,2*\dx);
    \coordinate (BR) at (1.35*\dx,-2*\dx);

    \coordinate (BLinner) at (-1.35*\dx, -\dx); 
    \coordinate (BRinner) at (1.35*\dx, -\dx);

    \coordinate (TLinner) at (-1.35*\dx, \dx);
    \coordinate (TRinner) at (1.35*\dx, \dx);

    \draw[fill=orange] (BLinner) -- (BL) to[out=270,in=270] (BR) -- (BRinner);

    \draw[fill=red] (TLinner) -- (TL) to[out=90,in=90] (TR) -- (TRinner);

    \filldraw[color=red, fill = red, path fading = south] (BRinner) -- (BLinner) -- (TLinner) -- (TRinner);
    \filldraw[color=orange, fill = orange, path fading = north] (BRinner) -- (BLinner) -- (TLinner) -- (TRinner);

    \draw[color=black] (-1.35*\dx, \dx+.1*\dx) -- (-1.35*\dx, -\dx-.1*\dx);
    \draw[color=black] (1.35*\dx, \dx+.1*\dx) -- (1.35*\dx, -\dx-.1*\dx);
\end{tikzpicture}}

==> results/Temps.tex <==
\pgfplotsset{every axis/.append style={thick,tick style={major tick
            length=4pt,thick,black}}}

\pgfkeys{/pgfplots/x axis shift down/.style={
        x axis line style={yshift=-#1},
        xtick style={yshift=-#1},
        tick align=outside,
        xticklabel shift={#1}}}

\pgfkeys{/pgfplots/y axis shift left/.style={
        y axis line style={xshift=-#1},
        ytick style={xshift=-#1},
        yticklabel shift={#1},
        scaled y ticks = false,
        tick align=outside,
        y tick label style={/pgf/number format/fixed,
        }
    }
}

\pgfplotsset{myPlot/.style={%
        line width = 1pt,
        separate axis lines,
        axis x line*=bottom,
        x axis shift down = 3pt,
        enlarge x limits=false,
        axis y line*=left,
        y axis shift left = 6pt,
        enlarge y limits={abs=.5pt},
        enlarge x limits={abs=.5pt},
        yticklabel shift={5pt},
    }
}

\input{results/myColors}

\pgfplotsset{resultsPlot/.style={%
	myPlot,
	const plot,
	height = 2.8cm,
	width = 8.4cm,
	xmin = 0,
	xmax = 180,
	xtick = {0, 30, ..., 180},
	%minor xtick= {1,3,5,7,...,97},
	xticklabels = {0, 0.5, ..., 3},
	grid=major,
  	grid style={black,line width=0.1pt,opacity=0.3},
	clip=true,  
    legend columns=4,
    legend style={
      at={(0.5, 1)},
      anchor=south,
      draw=none,
      fill=none,
      legend cell align=left,
      %/tikz/every even column/.append style={column sep=0.2cm}
      },
  	title style={
  		at={(0.5, 1.15)},
  		anchor=north,
  	},
	},
	tick label style={font=\small},
	label style={font=\small},
	%legend style={font=\footnotesize},
        legend style={row sep=0.55cm}
	}

\pgfplotsset{limit/.style = {const plot, color=black, dash pattern=on 1pt off 3pt on 3pt off 3pt, thick}}
\newcommand{\PlotVerticalLine}[1]{%
  \addplot[limit, forget plot, line width=1pt] plot coordinates{
    (#1,0)
    (#1,100)
  };
}

\newcommand{\Nstep}{60}

\begin{tikzpicture}
    
        \begin{axis}[
            resultsPlot,
            ylabel={$[10^3\cdot \text{kg}]$},
            ymin = 22.5,
            ymax = 25.1,
            xticklabels = {~},]

            \addplot [color=myOrangeA,  line legend, line width=1.5pt] table [x=time, y=x_sol_1, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\addplot [sharp plot,color=myGreenA, line legend] coordinates {(0,0) (0,0)};
            %\addplot [sharp plot,color=myOrangeB, dashed, line legend] coordinates {(0,0) (0,0)};
            %\addplot [sharp plot,color=myOrangeC, dashed, line legend] coordinates {(0,0) (0,0)};

            %\addplot [sharp plot,color=myRedA, line legend] coordinates {(0,0) (0,0)};
            %\addplot [sharp plot,color=myRedB, dotted, line legend] coordinates {(0,0) (0,0)};

            %\addplot [sharp plot,color=myOrangeD,  line legend] coordinates {(0,0) (0,0)};
            %\addplot [sharp plot,color=myRedC, dashed, line legend] coordinates {(0,0) (0,0)};

            %\addplot [color=black,  line legend, dashed, line width=1.pt] table [x=time, y=hat_x_8, col sep=comma] {results/results_QIHMPC_101023.csv};
            %\addplot [color=black,  line legend, dashed, line width=1.pt] table [x=time, y=hat_x_16, col sep=comma] {results/results_QIHMPC_101023.csv};

            \addlegendentry{$m_{\mathrm{v},1}(t)$} 
            \addlegendentry{$m_{\mathrm{v},6}(t)$} 

            \addplot [color=black,  line legend, dashed, line width=.7pt] table [x=time, y=hat_x_1, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}

        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -2.1cm)},
            %tick label style={font=\small, color=myOrangeA},
            %  y axis line style={myOrangeA},
            %  y tick style={myOrangeA},
            ymin = 19.,
            ymax = 33.5,
            ylabel={$[\text{kg}/\text{s}]$},
            xticklabels = {~},]

            \addplot [color=myOrangeB, dashed, line legend, line width=1.5pt] table [x=time, y=u_sol_1, col sep=comma] {results/results_QIHMPC_151023.csv};
            \addplot [color=myOrangeC, dashed, line legend, line width=1.5pt] table [x=time, y=u_sol_2, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\addplot [sharp plot,color=myGreenB, dashed, line legend] coordinates {(0,0) (0,0)};
            %\addplot [sharp plot,color=myGreenC, dashed, line legend] coordinates {(0,0) (0,0)};

            \addlegendentry{$q_{\mathrm{e},1}(t)$} 
            \addlegendentry{$q_{\mathrm{e},2}(t)$} 

            \addplot [color=black,  line legend, dashed, line width=.7pt] table [x=time, y=hat_u_1, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -4.2cm)},
            ylabel={$[10^3\cdot \text{kg}]$},
            ymin = 13.5,
            ymax = 16,
            xticklabels = {~},]

            \addplot [color=myGreenA,  line legend, line width=1.5pt] table [x=time, y=x_sol_2, col sep=comma] {results/results_QIHMPC_151023.csv};

            \addlegendentry{$m_{\mathrm{v},6}(t)$}

            \addplot [color=black,  line legend, dashed, line width=.7pt] table [x=time, y=hat_x_2, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}

            \end{axis}

            \begin{axis}[
            resultsPlot,
            shift={(0cm, -6.3cm)},
            ymin=4,
            ymax=11,
            ylabel={$[\text{kg}/\text{s}]$},
            xticklabels = {~},]

            \addplot [color=myGreenB, dashed, line legend, line width=1.5pt] table [x=time, y=u_sol_5, col sep=comma] {results/results_QIHMPC_151023.csv};
            \addplot [color=myGreenC, dashed, line legend, line width=1.5pt] table [x=time, y=u_sol_4, col sep=comma] {results/results_QIHMPC_151023.csv};

            \addlegendentry{$q_{\mathrm{e},7}(t)$} 
            \addlegendentry{$q_{\mathrm{e},8}(t)$}

            \addplot [color=black,  line legend, dashed, line width=.7pt] table [x=time, y=hat_u_5, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}

        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -8.4cm)},
            ymin=71.5,
            ymax=79.1,
            ylabel={$[^\circ\text{C}]$},
            xticklabels = {~},
            legend columns=5,]

            \addplot [color=myRedA,  line legend, line width=1.5pt] table [x=time, y=x_sol_8, col sep=comma] {results/results_QIHMPC_151023.csv};
            \addplot [color=myRedB,  line legend, dotted, line width=1.5pt] table [x=time, y=x_sol_16, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\addplot [sharp plot,color=myOrangeC, line legend] coordinates {(0,0) (0,0)};
            %  \addplot [sharp plot,color=myOrangeA, dotted, line legend] coordinates {(0,0) (0,0)};
            %  \addplot [sharp plot,color=myOrangeB, dotted, line legend] coordinates {(0,0) (0,0)};

            \addlegendentry{$T_{\mathrm{v},6}(t)$} 
            \addlegendentry{$T_{\mathrm{e},7}(t)$} 

            \addplot [color=black,  line legend, dashed, line width=.7pt] table [x=time, y=hat_x_8, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}

        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -10.5cm)},
            ymin = 1.0,
            ymax = 1.35,
            ylabel={$[\text{MW}]$},
            xticklabels = {~},]

            %\addplot [sharp plot,color=myRedC, dashed, line legend] coordinates {(0,0) (0,0)};
            \addplot [color=myRedC,  line legend, line width=1.5pt] table [x=time, y=u_sol_7, col sep=comma] {results/results_QIHMPC_151023.csv};

            \addlegendentry{$P_{\mathrm{pr},2}(t)$} 

            \addplot [color=black,  line legend, dashed, line width=.7pt] table [x=time, y=hat_u_7, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}

        \end{axis}
      
        \begin{axis}[
            resultsPlot,
            shift={(0cm, -12.6cm)},
            ymin = 43.,
            ymax = 47,
            ylabel={$[^\circ\text{C}]$},
            xticklabels = {~},]

            \addplot [color=myOrangeC,  line legend, line width=1.5pt] table [x=time, y=x_sol_3, col sep=comma] {results/results_QIHMPC_151023.csv};
            \addplot [color=myOrangeA,  line legend, dotted, line width=1.5pt] table [x=time, y=x_sol_10, col sep=comma] {results/results_QIHMPC_151023.csv};

            \addlegendentry{$T_{\mathrm{v},1}(t)$} 
            \addlegendentry{$T_{\mathrm{e},1}(t)$} 

            \addplot [color=black,  line legend, dashed, line width=.7pt] table [x=time, y=hat_x_3, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}

        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -14.7cm)},
            ymin=3.2,
            ymax=4.15,
            ylabel={$[\text{MW}]$},
            xlabel={Time $[\text{h}]$},]
        
            \addplot [color=myOrangeB,  line legend, line width=1.5pt] table [x=time, y=u_sol_6, col sep=comma] {results/results_QIHMPC_151023.csv};
        
            \addlegendentry{$P_{\mathrm{pr},1}(t)$} 

            \addplot [color=black,  line legend, dashed, line width=.7pt] table [x=time, y=hat_u_6, col sep=comma] {results/results_QIHMPC_151023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        
        \end{axis}

    \end{tikzpicture}

==> results/plotResults_QIHMPC_all_old.tex <==
\pgfplotsset{every axis/.append style={thick,tick style={major tick
            length=8pt,thick,black}}}

\pgfkeys{/pgfplots/x axis shift down/.style={
        x axis line style={yshift=-#1},
        xtick style={yshift=-#1},
        tick align=outside,
        xticklabel shift={#1}}}

\pgfkeys{/pgfplots/y axis shift left/.style={
        y axis line style={xshift=-#1},
        ytick style={xshift=-#1},
        yticklabel shift={#1},
        scaled y ticks = false,
        tick align=outside,
        y tick label style={/pgf/number format/fixed,
        }
    }
}

\pgfplotsset{myPlot/.style={%
        line width = 1pt,
        separate axis lines,
        axis x line*=bottom,
        x axis shift down = 3pt,
        enlarge x limits=false,
        axis y line*=left,
        y axis shift left = 6pt,
        enlarge y limits={abs=.5pt},
        enlarge x limits={abs=.5pt},
    }
}

\input{results/myColors}

\pgfplotsset{limit/.style = {const plot, color=black, dash pattern=on 1pt off 3pt on 3pt off 3pt, thick}}

\pgfplotsset{resultsPlot/.style={%
	myPlot,
	%const plot,
	height = 2.5cm,
	width = 8.4cm,
	xmin = 0,
	xmax = 180,
	xtick = {0, 30, ..., 180},
	%minor xtick= {1,3,5,7,...,97},
	xticklabels = {0, .5, ..., 3},
	grid=major,
  	grid style={black,line width=0.1pt,opacity=0.3},
	clip=true,  
    legend columns=4,
    legend style={
      at={(0.5, 1)},
      anchor=south,
      draw=none,
      fill=none,
      legend cell align=left,
      /tikz/every even column/.append style={column sep=0.3cm}
      },
  	title style={
  		at={(0.5, 1.15)},
  		anchor=north,
  	},
	},
	tick label style={font=\small},
	label style={font=\small},
	legend style={font=\footnotesize},
	}

    \pgfplotsset{limit/.style = {const plot, color=black, dash pattern=on 1pt off 3pt on 3pt off 3pt, thick}}
\newcommand{\PlotVerticalLine}[1]{%
  \addplot[limit, forget plot, line width=1pt] plot coordinates{
    (#1,0)
    (#1,100)
  };
}

    \newcommand{\Nstep}{90}

    \begin{tikzpicture}
    
        \begin{axis}[
            resultsPlot,
            ylabel={$[10^3\cdot \text{kg}]$},
            ymin = 22.5,
            ymax = 25.1,
            xticklabels = {~},]

            \addplot [color=Blue,  line legend, line width=1.5pt] table [x=time, y=x2_sol_1, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=RedOrange,  line legend, dashed, line width=1.5pt] table [x=time, y=x1_sol_1, col sep=comma] {results/results_QIHMPC_251023.csv};

            \addlegendentry{$m_{\mathrm{v},1}^{\mathrm{MPC1}}$} 
            \addlegendentry{$m_{\mathrm{v},6}^{\mathrm{MPC2}}$} 

            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_x_1, col sep=comma] {results/results_QIHMPC_251023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}

        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -1.9cm)},
            ymin = 18.,
            ymax = 34.,
            ylabel={$[\text{kg}/\text{s}]$},
            xticklabels = {~},]

            \addplot [color=BlueGreen, dashed, line legend, line width=1.5pt] table [x=time, y=u2_sol_1, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=BlueViolet, dashed, line legend, line width=1.5pt] table [x=time, y=u2_sol_2, col sep=comma] {results/results_QIHMPC_251023.csv};

            \addlegendentry{$q_{\mathrm{e},1}^{\mathrm{MPC1}}$} 
            \addlegendentry{$q_{\mathrm{e},2}^{\mathrm{MPC1}}$}

            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_u_1, col sep=comma] {results/results_QIHMPC_251023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -3.8cm)},
            ymin = 18.,
            ymax = 34,
            ylabel={$[\text{kg}/\text{s}]$},
            xticklabels = {~},]

            \addplot [color=Peach, dashed, line legend, line width=1.5pt] table [x=time, y=u1_sol_1, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=RubineRed, dashed, line legend, line width=1.5pt] table [x=time, y=u1_sol_2, col sep=comma] {results/results_QIHMPC_251023.csv};

            \addlegendentry{$q_{\mathrm{e},1}^{\mathrm{MPC2}}$} 
            \addlegendentry{$q_{\mathrm{e},2}^{\mathrm{MPC2}}$} 

            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_u_1, col sep=comma] {results/results_QIHMPC_251023.csv};

            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -5.7cm)},
            ylabel={$[10^3\cdot \text{kg}]$},
            ymin = 13.5,
            ymax = 16,
            xticklabels = {~},]
        
            \addplot [color=myBlueA,  line legend, line width=1.5pt] table [x=time, y=x2_sol_2, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=myRedA,  dashed, line legend, line width=1.5pt] table [x=time, y=x1_sol_2, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            \addlegendentry{$m_{\mathrm{v},6}^{\mathrm{MPC1}}$}
            \addlegendentry{$m_{\mathrm{v},6}^{\mathrm{MPC2}}$}
        
            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_x_2, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        
            \end{axis}
        
            \begin{axis}[
            resultsPlot,
            shift={(0cm, -7.6cm)},
            ymin=4,
            ymax=11,
            ytick = {4,7,10},
            yticklabels = {4,7,10},
            ylabel={$[\text{kg}/\text{s}]$},
            xticklabels = {~},]
        
            \addplot [color=myBlueB, dashed, line legend, line width=1.5pt] table [x=time, y=u2_sol_5, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=myBlueC, dashed, line legend, line width=1.5pt] table [x=time, y=u2_sol_4, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            \addlegendentry{$q_{\mathrm{e},7}^{\mathrm{MPC1}}$} 
            \addlegendentry{$q_{\mathrm{e},8}^{\mathrm{MPC1}}$}
        
            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_u_5, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        
        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -9.5cm)},
            ymin=4,
            ymax=11,
            ytick = {4,7,10},
            yticklabels = {4,7,10},
            ylabel={$[\text{kg}/\text{s}]$},
            xticklabels = {~},]
        
            \addplot [color=myRedB, dashed, line legend, line width=1.5pt] table [x=time, y=u1_sol_5, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=myRedD, dashed, line legend, line width=1.5pt] table [x=time, y=u1_sol_4, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            \addlegendentry{$q_{\mathrm{e},7}^{\mathrm{MPC2}}$} 
            \addlegendentry{$q_{\mathrm{e},8}^{\mathrm{MPC2}}$}
        
            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_u_5, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        
        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -11.4cm)},
            ymin = 43.,
            ymax = 45.1,
            ytick = {43,44,45},
            yticklabels = {43,44,45},
            ylabel={$[^\circ\text{C}]$},
            xticklabels = {~},]
        
            \addplot [color=myOrangeC,  line legend, line width=1.5pt] table [x=time, y=x2_sol_3, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=myOrangeA,  dashed, line legend, line width=1.5pt] table [x=time, y=x1_sol_3, col sep=comma] {results/results_QIHMPC_251023.csv};
            %\addplot [color=myOrangeA,  line legend, dotted, line width=1.5pt] table [x=time, y=x1_sol_10, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            \addlegendentry{$T_{\mathrm{v},1}^{\mathrm{MPC1}}$} 
            \addlegendentry{$T_{\mathrm{v},1}^{\mathrm{MPC2}}$}
            %\addlegendentry{$T_{\mathrm{e},1}$} 
        
            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_x_3, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        
        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -13.3cm)},
            ymin=2.75,
            ymax=4.15,
            ylabel={$[\text{MW}]$},
            xticklabels = {~},]
        
            \addplot [color=Cyan,  line legend, line width=1.5pt] table [x=time, y=u2_sol_6, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=myOrangeB,  dashed, line legend, line width=1.5pt] table [x=time, y=u1_sol_6, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            \addlegendentry{$P_{\mathrm{pr},1}^{\mathrm{MPC1}}$} 
            \addlegendentry{$P_{\mathrm{pr},1}^{\mathrm{MPC2}}$} 
        
            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_u_6, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        
        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -15.2cm)},
            ymin=71.5,
            ymax=79.1,
            ytick = {72,75,78},
            yticklabels = {72,75,78},
            ylabel={$[^\circ\text{C}]$},
            xticklabels = {~},
            legend columns=5,]
        
            \addplot [color=myPurpleA,  line legend, line width=1.5pt] table [x=time, y=x2_sol_8, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=myPinkA,  dashed, line legend, line width=1.5pt] table [x=time, y=x1_sol_8, col sep=comma] {results/results_QIHMPC_251023.csv};
            %\addplot [color=myRedB,  line legend, dotted, line width=1.5pt] table [x=time, y=x1_sol_16, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            %\addplot [sharp plot,color=myOrangeC, line legend] coordinates {(0,0) (0,0)};
            %  \addplot [sharp plot,color=myOrangeA, dotted, line legend] coordinates {(0,0) (0,0)};
            %  \addplot [sharp plot,color=myOrangeB, dotted, line legend] coordinates {(0,0) (0,0)};
        
            \addlegendentry{$T_{\mathrm{v},6}^{\mathrm{MPC1}}$} 
            \addlegendentry{$T_{\mathrm{v},6}^{\mathrm{MPC2}}$} 
            %\addlegendentry{$T_{\mathrm{e},7}$} 
        
            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_x_8, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        
        \end{axis}

        \begin{axis}[
            resultsPlot,
            shift={(0cm, -17.1cm)},
            ymin = 1.0,
            ymax = 1.8,
            ytick = {1,1.4,1.8},
            yticklabels = {1,1.4,1.8},
            ylabel={$[\text{MW}]$},
            xlabel={Time $[\text{h}]$},
            xlabel shift = -8 pt,]
        
            %\addplot [sharp plot,color=myRedC, dashed, line legend] coordinates {(0,0) (0,0)};
            \addplot [color=myPurpleB,  line legend, line width=1.5pt] table [x=time, y=u2_sol_7, col sep=comma] {results/results_QIHMPC_251023.csv};
            \addplot [color=myPinkB,  dashed, line legend, line width=1.5pt] table [x=time, y=u1_sol_7, col sep=comma] {results/results_QIHMPC_251023.csv};

            \addlegendentry{$P_{\mathrm{pr},2}^{\mathrm{MPC1}}$} 
            \addlegendentry{$P_{\mathrm{pr},2}^{\mathrm{MPC2}}$} 
        
            \addplot [color=black,  line legend, dotted, line width=.7pt] table [x=time, y=hat_u_7, col sep=comma] {results/results_QIHMPC_251023.csv};
        
            %\PlotVerticalLine{\Nstep-30}
            %\PlotVerticalLine{\Nstep}
        
        \end{axis}

    \end{tikzpicture}
